Taming Performance Variability caused by Client-Side Hardware Configuration

Many online services running in datacenters are implemented using a microservice software architecture characterized by strict latency requirements. Consequently, this popular software paradigm is increasingly used for the performance evaluation of server systems. Due to the scale and complexity of datacenters, the evaluation of server optimization techniques is usually done on a smaller scale using a client-server model. Although the experimental details of the server side are excessively described in most publications, the client side is often ignored. This paper identifies the hardware configuration of the client side as an important source of performance variation that can affect the accuracy and the correctness of the conclusions of a study that analyzes the performance of microservices. This is partially attributed to the strict latency requirements of microservices and the small scale of the experimental environment. In this work we present, using a widely used online-service, several examples where the accuracy and the trends of the conclusions differ based on the configuration of the client-side. At the same time we show that the experimental evaluation time can be significantly affected by the hardware configuration of the client. All these provoke the discussion of the right way to configure the experimental environment for assessing the performance of microservices.

==> chapters/_02_taxonomy-old.tex <==
\section{Taxonomy of Experimental Methodology}
We attempt to make a taxonomy to clarify under which conditions the configuration of the client can affect the conclusions of the experimental evaluation and how. The taxonomy focuses on three aspects: 1) time sensitivity of workload generator, 2) choice of client side HW configuration and 3) relation between the response time of the evaluated benchmark and the overhead of the client side. 

\textbf{Time-sensitive vs time-insensitive workload generator:} Workload generators are software components responsible to 1) generate a representative workload for the application/benchmark to process and to 2) accurately measure the end to end latency (i.e., average, 99th). Common characteristics among workload generators include the load intensity which represents the arrival time of jobs and resource demands which represents characteristics like the type and size of a job. Depending on the job arrival model of a workload generator, it can be categorized as time sensitive or time insensitive. Time sensitive or closed-loop workload generators send new jobs once previous jobs have finished execution. Time insensitive or open-loop workload generators, send jobs independently of the completion of previous jobs. Since HW configuration can affect the wakeup time of the system, it can affect the time the client gets notified about the completion of a job resulting in an inaccurate analysis. In the case where the workload generator is time sensitive, the underlying hardware configuration should be fixed in order to eliminate any variability. 

\textbf{Client side HW configuration:} The client side HW configuration refers to different settings of the client’s side system like hyperthreading, turbo mode, c-states and cpu frequency. These types of settings affect the accuracy of the end-to-end measurements for time-insensitive workload generators. If the point of latency measurement is inside the workload generator then in the case of the arrival of a response, the system should first wake-up and ramp up its frequency before the workload generator is able to capture the end-to-end latency increasing in this way the response time. This inaccuracy is not a fallback of the design methodology as long as the client environment in the experimental evaluation matches the production environment.  
Due to the large scale of datacenters and web-based applications, researchers evaluate data center related optimizations on test clusters with few nodes before propagating the optimization to the rest of the infrastructure. In fact there are a number of different works that only use a single node for the experimental evaluation. In these cases the client should act as another node or another microservice in the datacenter for the analysis to be representative in terms of end to end latency. Thus the configuration and the point of measurement of the client should match the configuration and the point of measurement of the production environment. Since these types of analysis estimate the speedup of an optimization and ultimately guide the number of resources required to serve a target load (TCO), an inaccurate experimental environment may cause either overprovision or underprovision of resources.

\textbf{Response time of benchmark:} With the emerge of the microservice software paradigm based on which applications are decomposed to several interconnected smaller services, the QoS of latency critical applications like search and social network has reduced significantly from ms to us while the request rates requirements have remained the same. Hardware overheads that are negligible for monolithic applications are now detrimental for the performance of microservice-based applications. As a result, microservices are especially vulnerable to the overhead introduced by the configuration of the client side since it is in the same order as the response time of the microservice (i.e. 500 us). For example C-state transition overhead can take from 2us up to 150us depending on the processor and legacy DVFS takes several microseconds (i.e., 40us [iDVFs]). In the case of monolithic applications or microservice-based applications with higher response time the client side HW configuration shouldn’t affect significantly neither the trends or the accuracy. 
